DreaMo: Articulated 3D Reconstruction From A Single Casual Video

Articulated 3D reconstruction has valuable applications in various domains, yet it remains costly and demands intensive work from domain experts. Recent advancements in template-free learning methods show promising results with monocular videos. Nevertheless, these approaches necessitate a comprehensive coverage of all viewpoints of the subject in the input video, thus limiting their applicability to casually captured videos from online sources. In this work, we study articulated 3D shape reconstruction from a single and casually captured internet video, where the subject's view coverage is incomplete. We propose DreaMo that jointly performs shape reconstruction while solving the challenging low-coverage regions with view-conditioned diffusion prior and several tailored regularizations. In addition, we introduce a skeleton generation strategy to create human-interpretable skeletons from the learned neural bones and skinning weights. We conduct our study on a self-collected internet video collection characterized by incomplete view coverage. DreaMo shows promising quality in novel-view rendering, detailed articulated shape reconstruction, and skeleton generation. Extensive qualitative and quantitative studies validate the efficacy of each proposed component, and show existing methods are unable to solve correct geometry due to the incomplete view coverage.

==> figure/recon_fine.tex <==
\begin{figure*}[ht!]
\begin{center}
\includegraphics[width=\textwidth]{figure/recon_fine_fig.pdf}
\end{center}
\vspace{-5pt}
\caption{
  \textbf{{\ourmethod} generates complete 3D shapes and renders plausible novel-view images.}
  The first column of each method is the rendered novel-view image and the second column is the reconstructed shape.
  %
  All the rendered images in a row correspond to the same object pose.
  \tao{try to merge fig4 and fig5.}
}
\label{fig:recon-fine}
\end{figure*}


==> figure/suppl_articulate_model.tex <==
\begin{figure*}[ht!]
\begin{center}
\includegraphics[width=\textwidth]{figure/suppl_articulate_model_fig.pdf}
\end{center}
\vspace{-1.5em}
\caption{
  \textbf{Manipulating {\ourmethod} by controlling the generated skeletons.}
  %
  We manually modify the bone positions and warp the associated skin to manipulate the reconstructed model into new poses.
}
\label{fig:suppl_articulate_model}
\end{figure*}


==> figure/suppl_dataset.tex <==
\begin{figure}[ht!]
\begin{center}
\includegraphics[width=.92\linewidth]{figure/suppl_dataset_fig.pdf}
\end{center}
\vspace{-1.2em}
\caption{
  Our self-collected video dataset for diverse species and insufficient view coverage from the Internet.
  %
  We present some cropped images from the entire dataset.
}
\label{fig:suppl_dataset}
\end{figure}


==> figure/suppl_network_arch.tex <==
\begin{figure*}[ht]
\begin{center}
\includegraphics[width=\textwidth]{figure/suppl_network_arch_fig.pdf}
\end{center}
\vspace{-1.5em}
\caption{
  \textbf{Network architecture of {\ourmethod}.}
  %
  We present the network design of the canonical implicit model (left), the blending models (upper right), and the global transformation model (lower right).
  %
  The warping models, which transform 3D coordinates between canonical and observation spaces, integrate blending and global transformation models, as elaborated in Section 3.1.
}
\label{fig:suppl_network_arch}
\end{figure*}


==> figure/suppl_reconst_results.tex <==
\begin{figure*}[ht!]
\begin{center}
\includegraphics[width=\textwidth]{figure/suppl_reconst_results_fig.pdf}
\end{center}
\vspace{-1em}
\caption{
  \textbf{3D reconstruction comparison among BANMo~\cite{yang2022banmo} and our {\ourmethod}.}
  %
  We show three rendered novel-view images, including RGB and depth, and their corresponding reconstructed shapes for each method.
}
\label{fig:suppl_reconst_results}
\end{figure*}


==> figure/teaser.tex <==
\begin{figure*}[ht]
\begin{center}
\includegraphics[width=.98\textwidth]{figure/teaser_fig.pdf}
\end{center}
\vspace{-10pt}
\caption{
  TBD
}
\label{fig:teaser}
\end{figure*}


==> section/3_approach_prev.tex <==
\section{Approach}
\label{sec:approach}
% TODO: \\
% (1) Preliminary: nerf, zero-1-to-3 \\
% (2) Our framework \\
% \indent * banmo \\
% \indent * novel view guidance \\
% \indent * regularization
\input{figure/method}
%%
\hubert{
We focus on the problem of non-rigid 3D shape reconstruction from a single video, where the recovered 3D shape is deformable and carries the time-dependent motions performed in the video.
% 
Our {\ourmethod} learns rest-pose neural 3D model represented by a neural implicit function in the time-invariant canonical space, while a separate time-dependent warping implicit function deforms the canonical space features to the observation space.
% 
Finally, we render 2D perspective images with the observation space features using volume rendering~\cite{mildenhall2021nerf}.
% 
We start by introducing the symbols of these functions in Section~\ref{} and Section~\ref{}, the diffusion prior in Section~\ref{}, the proposed loss functions in Section~\ref{}, then the skeleton generation algorithm in Section~\ref{}. 
}

\comment{
Given a single video capturing a non-rigid target object, we aim to reconstruct the target object's 3D shape and appearance.
%
To achieve this, our proposed framework, {\ourmethod}, learns a rest-pose neural 3D model represented by neural implicit functions~\cite{mildenhall2021nerf} in a time-invariant canonical space.
%
The 3D model in canonical space can be deformed to the observation space at each time step by a learned warping and be rendered to 2D using volume rendering~\cite{mildenhall2021nerf}.
}


%%
We unfold this section by first reviewing preliminary knowledge and then providing a detailed introduction to our proposed framework, {\ourmethod}.

\subsection{Preliminaries}
\label{sec:approach-preliminary}
\innersec{View-Conditioned 2D Diffusion Model.}
%%
2D diffusion models~\cite{} have demonstrated promising outcomes in generating realistic images through training on extensive datasets~\cite{}.
%
To integrate viewpoint control into the 2D diffusion models, Zero-1-to-3~\cite{liu2023zero123} finetunes StableDiffusion~\cite{} on a synthetic dataset~\cite{} with image pairs and their associated relative camera transformations.
%
It employs an image as a reference for the target object and generates the specific novel perspective of that object as defined by the input relative camera transformation.
%
Specifically, Zero-1-to-3 assumes that the object is positioned at the origin of the coordinate system, and the input camera transformation \(\mvec{\rho}=(\phi, \rho, r)\) denotes the relative azimuth, elevation, and camera distance, respectively.

\subsection{Neural Implicit Fields}
\label{sec:approach-neural-3d-field}
We represent the neural implicit 3D model in canonical space, with the 3D model assumed to be in a rest pose.
%
As in previous work~\cite{mildenhall2021nerf,yariv2021volsdf,yang2022banmo}, we model color \(\mvec{c}\), density \(\sigma\), and semantic feature \(\mvec{\xi}\) by neural implicit functions.
%
Specifically, they are predicted by Multilayer Perceptron networks (MLP) as follows:
%
\begin{align}
\label{eq:neural-3d-model-color}
\mvec{c} &= \mathrm{MLP}_{\mvec{\theta}_{c}}(\mvec{x}, \mvec{v}), \\
\label{eq:neural-3d-model-sdf}
d &= \mathrm{MLP}_{\mvec{\theta}_{d}}(\mvec{x}), \\
\label{eq:neural-3d-model-density}
\sigma &= \mathrm{\Phi}_{\beta}(-d), \\
\label{eq:neural-3d-model-feature}
\mvec{\xi} &= \mathrm{MLP}_{\mvec{\theta}_{\xi}}(\mvec{x}),
\end{align}
%
where \(\mvec{x}\) represents a 3D location in canonical space, \(\mvec{v}\) denotes a view direction, \(d\) is the signed distance function (SDF), \(\mathrm{\Phi}_{\beta}(\cdot)\) stands for the cumulative distribution function of the Laplacian distribution, utilized to convert the SDF to density~\cite{yariv2021volsdf}, and \(\beta\) is a learnable scale.

\subsection{Space Warping}
\label{sec:approach-warping}
We learn a forward warping \(\mathrm{warp}^{\text{fw}}_{t}(\cdot)\) to transition 3D points from canonical space to observation space at a specified time \(t\).
%
We also learn a backward warping function to \(\mathrm{warp}^{\text{bw}}_{t}(\cdot)\) execute the inverse operation.
%
Specifically, each warping is a composite of viewpoint transformation \(\mathrm{view}_{t}(\cdot)\) and object deformation \(\mathrm{deform}_{t}(\cdot)\).

%
\innersec{Object Deformation.} We apply neural blend skinning~\cite{yang2022banmo}, a skinning method inspired by linear blend skinning~\cite{skinningcourse-2014}.
%
By weighting the rigid motions \(\mathrm{\Delta}\mmat{J}_{b}\) of \(B\) bones, a point \(\mvec{x}^{*}\) in canonical space can be transformed from the rest pose to the corresponding location \(\mvec{x}^{*}_{t}\) for the pose at time \(t\) and vice versa:
%
\begin{align}
\label{eq:object-deform-forward}
\mvec{x}^{*}_{t} &= \mathrm{deform}^{\text{fw}}_{t}(\mvec{x}^{*}) = \sum_{b}{\mvec{w}^{\text{fw}}_{b}}\mathrm{\Delta}\mmat{J}^{t}_{b}\,\mvec{x}^{*}, \\
\label{eq:object-deform-backward}
\mvec{x}^{*} &= \mathrm{deform}^{\text{bw}}_{t}(\mvec{x}^{*}_{t}) = \sum_{b}{\mvec{w}^{\text{bw}}_{b}}(\mathrm{\Delta}\mmat{J}^{t}_{b})^{-1}\mvec{x}^{*}_{t},
\end{align}
where \(\mathrm{\Delta}\mmat{J}^{t}_{b} = \mmat{J}^{t}_{b}\,(\mmat{J}^{*}_{b})^{-1}\), \(\mmat{J}^{t}_{b}\) and \(\mmat{J}^{*}_{b}\) denotes the rigid transformations of the \(b\)-th bone from "zero-configuration" to the pose at time \(t\) and the rest pose, respectively, and \(\mmat{w}^{t}\in\mathbb{R}^{B}\) is the skinning weights which we describe later.
% Move to implementation
In practice, \(\mmat{J}^{t}_{b}=\mathrm{MLP}_{\mvec{\theta}_{p}}(\mvec{e}^{t}_{b})\) and \(\mmat{J}^{*}_{b}=\mathrm{MLP}_{\mvec{\theta}_{p}}(\mvec{e}^{*}_{b})\), where \(\mvec{e}^{t}_{b}\) and \(\mvec{e}^{*}_{b}\) are latent pose embedding.

\innersec{Skinning Weights.}
Inspired by prior work~\cite{yang2022banmo, yang2021lasr}, we implicitly represent a bone by a Gaussian ellipsoid.
%
The skinning weight \(\mvec{w}_{b}\) for a point \(\mvec{x}\) to the \(b\)-th bone is determined by the Mahalanobis distance between \(\mvec{x}\) and the \(b\)-th Gaussian ellipsoid.
%
By applying softmax to the distances from the specified point \(\mvec{x}\) to \(B\) bones, we obtain the skinning weights \(\mvec{w}_{b}\).
%
In practice, by converting \(\mvec{x}\) to the \(b\)-th bone's coordinate, defined by \(\mmat{J}_{b}\), and scaling each axis in the bone's coordinate by a learnable Gaussian scale, we can determine the Mahalanobis distance by examining the difference between the transformed point and the origin.

% %
% \begin{equation}
% \label{eq:skinning-weight}
% \begin{split}
% \mvec{w}_{b}={(\mvec{x}-\mvec{\mu}_{b})}^{T}\mmat{Q}_{b}(\mvec{x}-\mvec{\mu}_{b}),
% \end{split}
% \end{equation}
% where \(\mmat{Q}_{b}=\sum_{i=1}^{3}\frac{1}{\lambda_{i, b}}\mvec{v}_{i,b}{(\mvec{v}_{i,b})}^{T}\) is the precision matrix that is determined by a learnable orientation \(\mvec{v}_{i, b}\) and a learnable scale \(\lambda_{i, b}\) of the Gaussian, and \(\mvec{\mu}_{b}\) is a learnable center of the Gaussian.

%
\innersec{Viewpoint Transformation.} A camera pose \(\mmat{P}_t\in\mathrm{SE}(3)\) is learned for each time step \(t\).
%
The viewpoint transformation between a 3D location \(\mvec{x}^{*}_{t}\) in canonical space and its corresponding location \(\mvec{x}_{t}\) in the observation space at time \(t\) can be derived using:
%
\begin{align}
\label{eq:view-transform-forward}
\mvec{x}_{t} &= \mathrm{view}^{\text{fw}}_{t}(\mvec{x}^{*}_{t}) = \mmat{P}_t\mvec{x}^{*}_{t}, \\
\label{eq:view-transform-backward}
\mvec{x}^{*}_{t} &= \mathrm{view}^{\text{bw}}_{t}(\mvec{x}_{t}) = \mmat{P}_t^{-1}\mvec{x}_{t}.
\end{align}

Finally, the formulation for forward and backward warping for the mapping between \(\mvec{x}^{*}\) in canonical space with rest pose and \(\mvec{x}_{t}\) in observation space can be derived as follows
\begin{equation}
\label{eq:warping}
\begin{split}
\mathrm{warp}^{\text{fw}}_{t}(\mvec{x}^{*}) &= \mathrm{view}^{\text{fw}}_{t}(\mathrm{deform}^{\text{fw}}_{t}(\mvec{x}^{*})), \\
\mathrm{warp}^{\text{bw}}_{t}(\mvec{x}_{t}) &= \mathrm{deform}^{\text{bw}}_{t}(\mathrm{view}^{\text{bw}}_{t}(\mvec{x}_{t})).
\end{split}
\end{equation}

% %
% A rigid motion \(\mathrm{\Delta}J_{b}\) can be obtained by 

% The rigid motions \(J^{t}_b=\mathrm{MLP}_{\theta_{a}}(\mvec{w}^{t}_{b})\) of \(B\) bones are predicted from a latent body pose embedding \(\mvec{w}^{t}_{b}\).


\subsection{View-Conditioned Diffusion Model as Prior}
\label{sec:approach-view-prior}
To address the challenge of missing viewpoints in the input video, we employ Zero-1-to-3~\cite{liu2023zero123}, a pretrained 2D diffusion model for novel view synthesis, as a prior.
%
We apply the Score Distillation Sampling (SDS)~\cite{poole2022dreamfusion} to transfer novel-view knowledge from Zero-1-to-3 to \ourmethod.

%
Zero-1-to-3 is equipped with a learned noise prediction function \(\epsilon_{\mvec{\phi}}(\mvec{z}_{i}; \mvec{\rho},i)\) that predicts the sampled noise \(\mvec{\epsilon}\) given the noisy image \(\mvec{z}_{i}\) at a noise level \(i\) and a relative camera transformation \(\mvec{\rho}\) describing the camera azimuth, elevation, and distance.
%
It provides the gradient direction for updating {\ourmethod} in a manner that guides all rendered images towards the high probability density regions, conditioned on the relative camera transformation under the diffusion prior:
%
\begin{equation}
\label{eq:diffusion-prior}
\mathrm{\Delta}\mathcal{L}_{\text{sds}}(\mvec{\phi}, \mvec{y})=\expect_{t, \mvec{\epsilon}}\left[w(t)\left(\epsilon_{\mvec{\phi}}(\mvec{z}_{i}; \mvec{\rho},i)-\mvec{\epsilon}\right)\frac{\partial\mvec{y}}{\partial\mvec{\theta}}\right],
\end{equation}
%
where \(w(t)\) denotes a weighting function, \(\mvec{y}\) represents the rendered image at a novel view with the same camera pose as \(\mvec{\rho}\) by {\ourmethod}, and \(\mvec{\theta}\) stands for the parameters of {\ourmethod}.
%
In practice, we observe that exclusively updating parameters associated with articulation (\(\mvec{\theta}_{p}\) and \(\mvec{e}^{t}_{b}\)) is adequate to reconstruct the target object and prevents texture artifacts resulting from the imperfect diffusion prior.

\subsection{Rendering}
\label{sec:approach-rendering}
We apply volume rendering~\cite{yang2022banmo, mildenhall2021nerf} to render an image.
%
to obtain the rendered value of a 2D pixel \(\mvec{u}\) at time \(t\), an array of 3D points \(\mvec{x}_{i}\) are sampled along a camera ray cast from \(\mvec{u}\).
%
The rendered color \(\mvec{c}(\mvec{u})\), feature \(\mvec{\xi}(\mvec{u})\), and opacity \(o(\mvec{u})\) are then computed by weighting over the neural 3D field functions (Section~\ref{sec:approach-neural-3d-field}) of the corresponding warped 3D points \(\mvec{x}^{*}_{i}=\mathrm{warp}^{\mathrm{bw}}_{t}(\mvec{x}_{i})\):
%
\begin{align}
\label{eq:vol-render}
\mvec{c}(\mvec{u}) &= \sum_{i}\tau_{i}\mvec{c}(\mvec{x}^{*}_{i}), \\
\mvec{\xi}(\mvec{u}) &= \sum_{i}\tau_{i}\mvec{\xi}(\mvec{x}^{*}_{i}), \\
o(\mvec{u}) &= \sum_{i}\tau_{i},
\end{align}
where \(\tau_{i}=\mathrm{\Pi}_{j=1}^{i-1}p_j(1-p_i)\), and \(p_i=\exp{(-\sigma(\mvec{x}^{*}_{i})\delta_{i})}\) denotes the probability that a photon passes through the interval \(\delta_{i}\) between \(\mvec{x}_i\) and its subsequent sample \(\mvec{x}_{i+1}\).

%%
To render the 2D optical flow, we warp the ray points \(\mvec{x}_i\) from the pixel \(\mvec{u}_t\) at time \(t\) to the target time \(t'\), and compute the expected 2D projection location
\begin{equation}
\label{eq:optical-flow}
\mvec{u}_{t'} = \sum_{i}\tau_i\mathrm{\Pi}^{t'}\left(\mathrm{warp}^{\mathrm{fw}}_{t'}\left(\mathrm{warp}^{\mathrm{bw}}_{t}(\mvec{x}_{i})\right)\right).
\end{equation}
Then, the optical flow is derived by \(\mvec{f}_{t \to t'}(\mvec{u}_{t})=\mvec{u}_{t'}-\mvec{u}_{t}\).

\subsection{Learning}
Our overall loss combining reconstruction, SDS, and regularization can be expressed as follows:
%
\begin{equation}
\label{eq:total-loss}
\begin{split}
\mathcal{L}_{\text{total}}=&w_{\text{recon}}\mathcal{L}_{\text{recon}} + w_{\text{sds}}\mathcal{L}_{\text{sds}} + w_{\text{ncyc}}\mathcal{L}_{\text{ncyc}} \\
+ &w_{\text{surf}}\mathcal{L}_{\text{surf}} + w_{\text{smooth}}\mathcal{L}_{\text{smooth}}.
\end{split}
\end{equation}
%
Next, we elaborate on each loss term.

\label{sec:approach-learning}
\innersec{Reconstruction Loss.}
The reconstruction loss empowers {\ourmethod} to build the 3D model by minimizing discrepancies between the appearance \(\mvec{c}'(\mvec{u})\), semantic feature \(\mvec{\xi}'(\mvec{u})\), silhouette \(o'(\mvec{u})\), optical flow \(\mvec{f}'_{t \to t'}(\mvec{u})\), and their respective rendered outputs:
%
\begin{equation}
\begin{split}
\label{eq:reconstruction-loss}
\mathcal{L}_{\text{recon}} &= \frac{1}{M}\sum_{\mvec{u}}
\norm{\mvec{c}'(\mvec{u}) - \mvec{c}(\mvec{u})}{2} +
\norm{\mvec{\xi}'(\mvec{u}) - \mvec{\xi}(\mvec{u})}{2} \\
&+ \norm{o'(\mvec{u}) - o(\mvec{u})}{2} +
\norm{\mvec{f}'_{t \to t'}(\mvec{u}) - \mvec{f}_{t \to t'}(\mvec{u})}{2},
\end{split}
\end{equation}
%
where $M$ is the number of pixels in a batch.

%%
\innersec{Regularization.} To encourage the inverse relationship between the forward and backward warpings, we employ the novel-view warping cycle loss.
%
\begin{equation}
\label{eq:reg-warp-consistency}
\mathcal{L}_{\text{ncyc}} = \sum_{i}\tau_{i}\norm{\mvec{x}_{i} - \mathrm{warp}^{\text{fw}}_{t}(\mathrm{warp}^{\text{bw}}_{t}(\mvec{x}_{i}))}{2},
\end{equation}
%
where \(\mvec{x}_{i}\) is a ray point on a sampled camera ray.
%
Rather than solely sampling rays on training views~\cite{yang2022banmo}, we propose sampling rays on unseen views as well.

%%
Intuitively, the Gaussian bones should be within the surface and smoothly change over time.
%
To constrain the bones to locate within surface, we introduce the within-surface loss \(\mathcal{L}_{\text{surf}}\) on the SDF values \(d=\mathrm{MLP}_{\mvec{\theta_{d}}}(\mvec{x}^{*})\) of sampled canonical points \(\mvec{x}^{*}\):
%
\begin{equation}
\label{eq:reg-within-surface}
\mathcal{L}_{\text{surf}} = 
\begin{cases}
  \norm{d}{2} & \text{if \(d > 0\)} \\
  0 & \text{otherwise.}
\end{cases}
\end{equation}
%
To make the transition across time smooth, we propose the smooth transition loss:
\begin{equation}
\label{eq:reg-smooth-transition}
\begin{split}
\mathcal{L}_{\text{smooth}} = \frac{1}{B(T-1)}\sum^{B}_{b=1}\sum^{T-1}_{t=1}&(\mathrm{angle}(\mmat{R}^{t}_{b}, \mmat{R}^{t+1}_{b}) \\
&+ \norm{\mvec{t}^{t}_{b} - \mvec{t}^{t+1}_{b}}{2}),
\end{split}
\end{equation}
where \(\left(\mmat{R}^{t}_{b}|\mvec{t}^{t}_{b}\right)=\mmat{J}^{t}_{b}\), and the relative angle of two rotations can be computed by \(\mathrm{angle}(\mmat{R}_{1}, \mmat{R}_{2})=\arccos((\mathrm{tr}(\mmat{R}_{1}, \mmat{R}_{2}^{\intercal})-1)/2)\).

\subsection{Skeleton Generation}
\label{sec:approach-skeleton-gen}
The regularization techniques described above empower {\ourmethod} to learn human-interpretable Gaussian bones.
%
In this section, we elucidate how we generate a skeleton for a given target based on the learned Gaussian bones.
%
The core idea is to establish a connection between a pair of Gaussian bones when they exert the most significant impact, measured by skinning weights, on two adjacent sections of skin, respectively.

%%
To this end, we first extract the rest surface of the 3D model by running marching cubes with $128^3$ voxel grids, resulting in a 3D mesh $M=(V, S)$ with $N$ vertices $V = \{\mvec{v}_i \in \mathbb{R}^3\}_{i=1}^{N}$ and $N$ faces $S = \{\mvec{s}_i \in V^3\}_{i=1}^{N}$.
%
Subsequently, given $B$ Gaussian bones $\{b_i\}_{i=1}^{B}$, we assign each vertex $\mvec{v}_i \in V$ to a Gaussian bone $b_i$ that has the largest skinning weight of the vertex at rest pose. 
%
Following this, we traverse each face $\mvec{s} \in S$ and assign a connection to the pair of Gaussian bones $(b_j, b_k)$ if there exists a pair of vertices in $\mvec{s}$ that are assigned to $b_j$ and $b_k$, respectively.

